Improving Matrix Completion by Exploiting Rating Ordinality in Graph Neural Networks

Matrix completion is an important area of research in recommender systems. Recent methods view a rating matrix as a user-item bi-partite graph with labeled edges denoting observed ratings and predict the edges between the user and item nodes by using the graph neural network (GNN). Despite their effectiveness, they treat each rating type as an independent relation type and thus cannot sufficiently consider the ordinal nature of the ratings. In this paper, we explore a new approach to exploit rating ordinality for GNN, which has not been studied well in the literature. We introduce a new method, called ROGMC, to leverage Rating Ordinality in GNN-based Matrix Completion. It uses cumulative preference propagation to directly incorporate rating ordinality in GNN's message passing, allowing for users' stronger preferences to be more emphasized based on inherent orders of rating types. This process is complemented by interest regularization which facilitates preference learning using the underlying interest information. Our extensive experiments show that ROGMC consistently outperforms the existing strategies of using rating types for GNN. We expect that our attempt to explore the feasibility of utilizing rating ordinality for GNN may stimulate further research in this direction.

==> sections/0201method_old.tex <==
We present progressive \underline{P}reference \underline{D}ecomposition for \underline{G}NN-based \underline{MC} (\proposed) that exploits progressively decomposed graphs based on user preference (Figure \ref{fig:method}).
\proposed directly utilizes the inclusion relationships according to the ordinality of the ratings, unlike the prior methods treating rating types independently.

\subsection{Reflecting Rating Ordinality to GNN}
To reflect the ordinal nature of ratings in message passing, our method ensures that higher ratings are propagated more frequently. We introduce a cumulative message passing strategy.
Given the bipartite graph $G$, we decompose the graph into a set of unweighted subgraphs so that each decomposed graph progressively includes stronger relations from users’ general interest to high preferences. 
Each subgraph contains all the nodes, but different edges according to the degree of user preference.
First, we generate a graph $G_{I}$ by including all observed interactions (i.e., both $U$ and $\mathcal{R}$) to model users’ general interest. Unlike $G$, $G_I$ treats all relation types equally.
Second, we generate a set of subgraphs with different preference levels $\{G_{t}\}_{t\in \mathcal{T}}$ by collecting edges with ratings greater than or equal to $t$ into $G_t$, where $\mathcal{T}$ is the set of relation types used for the decomposition.
Edges that correspond to unknown ratings are excluded from $G_t$.
Note that when faced with a large rating scale (e.g., $R = 100$), unlike prior studies, our approach allows for a more spaced-out configuration of $\mathcal{T}$ (e.g., $\mathcal{T} = \{1,25,50,100\}$).
In this work, we use $\mathcal{R}$ as $\mathcal{T}$.

Then, we apply GNN to each graph $G_x$ to exploit the graph structure by propagating representations on it.
We follow the propagation rule of \cite{he2020lightgcn, inductiveMC_CIKM21} which has the following form:
\begin{equation}
\begin{aligned}
    e^{l+1}_x[i] = \sum_{j \in \mathcal{N}_x(i)} \frac{1}{c_{ij}} e^l_x[j],
\end{aligned}
\end{equation}
where $\mathcal{N}_x(i)$ denotes the set of node $i$'s neighbors in $G_x$, and 
$e^l_x[i]$ denotes node $i$’s representation in $G_x$.
After $L$ propagation layers, we aggregate the representations from each layer to form the representation $h_x[i]$ from each subgraph, i.e., $h_x[i] = AGG(\{e^l_x[i] \mid 0 \leq l \leq L\})$.
In sum, for each node $i$, we obtain $h_t[i]$ from each $G_{t}$ and $h_I[i]$ from $G_I$.



\textbf{Remarks.} 
Compared to the rating-wise decomposition \cite{inductiveMC_CIKM21}, our progressive decomposition provides more number of edges for each rating type, which can be interpreted as a kind of augmentation based on ordinality.
This enables a more effective propagation when user feedback does not exist sufficiently for all rating types.
Also, as edges with higher ratings are more frequently utilized in the propagation process, users' strong preferences are naturally more reflected in predictions.
We provide experiment results supporting the effectiveness of our decomposition strategy in Sec. \ref{sec:further}.


\subsection{Robust Propagation through Leveraging Unknown Ratings} 
**
As ratings are given only to a small fraction of user-item interactions, $\{G_{t}\}_{t\in \mathcal{T}}$ still has a high sparsity.
In particular, the subgraph with a higher preference level has a smaller number of edges.
To cope with the sparsity problem, we propose interest regularization that utilizes user's interest from $G_{I}$ to provide guidance to the learning user's preference from $\{G_{t}\}_{t\in \mathcal{T}}$.
As all ratings are given after the user tried an item and thus occur based on the same interest semantics, we make $\{h_{t}[i]\}_{t\in \mathcal{T}}$ to share the same semantic of user interest $h_{I}[i]$:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{IR} = \sum_{1 \leq i \leq N}\frac{1}{|\mathcal{T}|}\sum_{t\in \mathcal{T}} \big\lVert h_t[i] - h_I[i] \big\rVert_2
\end{aligned}
\end{equation}
where $N$ is the total number of users and items. 


\subsection{Bilinear Decoder}
Following \cite{GCMC, inductiveMC_CIKM21}, we use a bilinear decoder to predict links in the user-item graph.
We first make the final representation $h[i]$ of each node $i$ by accumulating $h_t[i]$ by sum operator \cite{inductiveMC_CIKM21}, i.e., $h[i]=\sum_{t \in \mathcal{T}} h_t[i]$.
Given the final representation $h[i]$ of user $i$ and $h[j]$ of item $j$, the decoder produces a probability distribution over the rating types through a bilinear operation:
\begin{equation}
\begin{aligned}
z^r_{ij} &= h[i]^{T} Q_{r} h[j]\\
p(\hat{M}_{ij}=r) &= \frac{\exp(z^r_{ij})}{\sum_{s \in \mathcal{R}}\exp(z^s_{ij})},
\end{aligned}
\end{equation}
where $\hat{M}_{ij}$ is the predicted rating and $Q_{r}$ is a trainable parameter matrix.
The final rating is computed by $\hat{M}_{ij} = \sum_{r \in \mathcal{R}} r \, p(\hat{M}_{ij}=r)$.



\subsection{Model Training}
As \proposed utilizes both preference (i.e. ratings) and interest (i.e., the existence of edges), we use pair-wise ranking loss \cite{BPR} along with the rating prediction loss \cite{GCMC, inductiveMC_CIKM21}.
This pair-wise loss trains the model to discriminate between observed and unobserved interactions, facilitating learning of user interest.
Let $\mathcal{D}=\{(i,j,k) \mid M_{ij} \in \mathcal{R} \land M_{ik} \not\in \mathcal{R} \cup \{U\}\}$ denote the set of training instances, i.e., user $i$ gives rating to item $j$ but doesn't interact with item $k$.
The loss function is defined as follows:
\begin{equation}
\begin{aligned}
\mathcal{L}=-\sum_{(i, j, k) \in \mathcal{D}} \left( 
\sum_{r\in \mathcal{R}} I(r=M_{ij}) \log p(\hat{M}_{ij}=r)
+
\alpha \log\sigma \left(o_{ij} - o_{ik} \right)
\right) 
\end{aligned}
\end{equation}
where the first term corresponds to the cross-entropy loss between the predictions and the ground-truth ratings \cite{GCMC, inductiveMC_CIKM21}, the second term is the pair-wise loss.
$I(\cdot)$ is the indicator function, $\alpha$ is a hyperparameter balancing the two terms, and $\sigma(\cdot)$ is the sigmoid function.
$o_{ij}$ denotes the interest score of user $i$ to item $j$.
We compute it by the sum of unnormalized scores, i.e., $o_{ij} = \sum_{r\in\mathcal{R}} z^r_{ij}$.
Finally, \proposed trains the model with the following loss function:
\begin{equation}
\begin{aligned}
\mathcal{L}_f= \mathcal{L} + \lambda \mathcal{L}_{IR}
\end{aligned}
\end{equation}
where $\lambda$ is a hyperparameter controlling the regularization effects.



\begin{equation}
\label{eq:RT}
\begin{aligned}
    e^{l+1}[i] = \sum_{j \in \mathcal{N}(i)} \frac{1}{c_{ij}} \mathbf{W}^l e^l[j],
\end{aligned}
\end{equation}

==> sections/034further_analysis2.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=1.\linewidth]{./images/sim_sole.png }
    \caption{Comparison of L2 distances between the average of user embeddings across various relationship types. (a) corresponds to GCMC+, and (b) corresponds to \proposed}
    \label{fig:further_analysis2}
    \vspace{-0.5cm}
\end{figure}
